Scalable PAC-Bayesian Meta-Learning via the PAC-Optimal Hyper-Posterior: From Theory to Practice

Meta-Learning aims to speed up the learning process on new tasks by acquiring useful inductive biases from datasets of related learning tasks. While, in practice, the number of related tasks available is often small, most of the existing approaches assume an abundance of tasks; making them unrealistic and prone to overfitting. A central question in the meta-learning literature is how to regularize to ensure generalization to unseen tasks. In this work, we provide a theoretical analysis using the PAC-Bayesian theory and present a generalization bound for meta-learning, which was first derived by Rothfuss et al. (2021a). Crucially, the bound allows us to derive the closed form of the optimal hyper-posterior, referred to as PACOH, which leads to the best performance guarantees. We provide a theoretical analysis and empirical case study under which conditions and to what extent these guarantees for meta-learning improve upon PAC-Bayesian per-task learning bounds. The closed-form PACOH inspires a practical meta-learning approach that avoids the reliance on bi-level optimization, giving rise to a stochastic optimization problem that is amenable to standard variational methods that scale well. Our experiments show that, when instantiating the PACOH with Gaussian processes and Bayesian Neural Networks models, the resulting methods are more scalable, and yield state-of-the-art performance, both in terms of predictive accuracy and the quality of uncertainty estimates.

==> content/abstract.tex <==
%\looseness -1 Due to their complex parameter space, choosing informative priors for Bayesian Neural Networks (BNNs) is challenging. Thus, often a naive, zero-centered Gaussian is used, resulting both in bad generalization and poor uncertainty estimates when training data is scare.
%
%In contrast, {\em meta-learning} aims to extract such prior knowledge from a set of related learning tasks. We propose a principled and scalable algorithm for meta-learning BNN priors based on PAC-Bayesian bounds. Whereas previous approaches require optimizing the prior and multiple variational posteriors in an interdependent manner, our method does not rely on difficult nested optimization problems and is agnostic to the variational inference method used. Our experiments show that the proposed method is not only computationally efficient but also yields better predictions and uncertainty estimates when compared to previous meta-learning methods and BNNs with standard priors.

==> content/lifelong.tex <==
\newpage
\section{PAC-Bayesian Meta-Learning for Sequential Decision-making}

We give an extension of Theorem~\ref{theorem:meta-learning-bound}, which supports offline meta-learning for sequential decision making.
Therefore, We no longer assume that the sample $S_i$ is i.i.d., which allows us to view $Q_i$ as an Bayesian sequential decision-making algorithm. Instead, we assume that within each task, the sample is history dependant, meaning that for all $i= 1, \dots, n$ and all $j= 1,\dots, m_i$, the input $x_j$ only depends on $(z_\tau)_{\tau < j}$. Similar to before, we assume that the tasks are drawn i.i.d.~from an environment $\calT$.


The goal is to show,
\begin{align*}
  \calL(\calQ, \calT) - \hat{\calL}(\calQ, S_1, \dots, S_n) 
  \leq & \left(\frac{1}{\lambda} + \frac{1}{n \beta}\right)D_{KL}(\calQ \vert\vert \calP) \\
  & + \frac{1}{n}\sum_{i=1}^n\E_{P \sim \calQ} D_{KL}(Q(S_i, P) \vert \vert P) + \mathrm{MGFs}.
\end{align*}

Following the proof of Theorem~\ref{theorem:meta-learning-bound}, we can apply the two change of measure inequalities as before. For bounding the MGFs however, we need to invoke Martingale concentration inequalities instead. We have,
\begin{align*}
  \calL(\calQ, \calT) - \hat{\calL}(\calQ, S_1, \dots, S_n) 
  \leq & \left(\frac{1}{\lambda} + \frac{1}{\gamma}\right)D_{KL}(\calQ \vert\vert \calP) \\
  & + \frac{1}{\gamma}\sum_{i=1}^n\E_{P \sim \calQ} D_{KL}(Q(S_i, P) \vert \vert P) + \Upsilon^{\mathrm{I}}(\gamma) + \Upsilon^{\mathrm{II}}(\lambda)
\end{align*}
where,
\begin{align*}
 \Upsilon^{\mathrm{I}}(\lambda) & = \ln\E_{P \sim \calP} \left[\exp\left( \frac{\lambda}{n}\sum_{i=1}^n \E_{\calD, S \sim \calT} \left( \calL(Q(P, S), D) - \calL(Q(P,S_i), \calD_i)\right)\right)\right]^{1/\lambda}\\
\Upsilon^{\mathrm{II}}(\gamma) & =  \ln\E_{P \sim \calP} \E_{h \sim P} \left[\exp\left( \frac{\gamma}{n}\sum_{i=1}^n  \left( \calL(h, D_i) - \calL(h, S_i)\right)\right)\right]^{1/\gamma} 
\end{align*}

We define $X_i = \calL(Q(P, S_i), D_i) - \frac{1}{n} \E_{\calD, S\sim \calT} \calL( Q(P, S), \calD)$ and $M_i = \sum_{j=1}^i X_j$. Then $M_i$ is a martingale sequence w.r.t the filteration $\calF = {S_1, S_2, \dots}$, since
\[
\E M_i \vert M_{i-1} = M_{i-1} + \E X_i \vert M_{i-1}
\]

% \paragraph{Tricky Setting: Life-Long Learning}
% We now consider the life-long setting in which a sequence of tasks are presented to the learner one after the other.
% Here the hyper-posterior, and in turn the priors, are updated sequentially, after the data from each new task is solved. For every task $i$, we use the base learner $Q_i = Q(S_i,P_i)$ where $P_i$ is the meta-learned prior. 

% Define the average loss after solving $n$ tasks as,
% \[
% \calL(\calQ_1, \dots,\calQ_n, \calT) \coloneqq \frac{1}{n}\sum_{i=1}^n \calL(\calQ_i, \calT) = \frac{1}{n} \sum_{i=1}^n \E_{P_i \sim \calQ_i} \Big( \E_{\calD\sim \calT} \E_{S\sim \calD}\big( \calL(Q(S, P_i), \calD)\big) \Big)
% \]
% And its empirical counterpart will be,
% \[
% \hat{\calL}(\calQ_1, \dots,\calQ_n, S_1, \dots, S_n) = \frac{1}{n} \sum_{i=1}^n \hat{\calL} (\calQ_i, S_i) = \frac{1}{n} \sum_{i=1}^n \E_{P_i \sim \calQ_i} \hat{\calL}(Q(S_i, P_i), S_i)
% \]

% The goal is to show,
% \begin{align*}
%   \calL(\calQ_1, \dots,\calQ_n, \calT) - \hat{\calL}(\calQ_1, \dots,\calQ_n, S_1, \dots, S_n) 
%   \leq & \left( \dots\right)\sum_{i=1}^n D_{KL}(\calQ_i \vert\vert \calP) \\
%   & + \E_{P_i \sim \calQ_i} D_{KL}(Q_i(S_i, P_i) \vert \vert P_i) + \mathrm{MGFs}.
% \end{align*}
% To this end we define,
% \[\tilde{\calL}(\calQ_1, \dots, \calQ_n, \calD_1, \dots, \calD_n) = \frac{1}{n} \sum_{i=1}^n \E_{P_i\sim\calQ_i} \Big( \E_{S, \calD_i} \calL(Q(S, P_i), \calD_i)\Big).\]

% Consider the function $\varphi_\mathrm{Meta}(P_1, \dots, P_n) \coloneqq \calL(P_1, \dots, P_n, \calT) - \tilde{\calL}(P_1, \dots, P_n, \calD_1, \dots, \calD_n)$. 
% Define $\rho = \prod_{i=1}^n \calQ_i$ and $\pi = \calP^n$. 
% Then by the change of measure inequality invoked for the tuple $(\varphi_{\mathrm{Meta}}(\cdot), \rho, \pi)$,
% \[
% \calL(\calQ_1, \dots,\calQ_n, \calT)  \leq  \tilde{\calL}(\calQ_1, \dots, \calQ_n, \calD_1, \dots, \calD_n) +\frac{1}{\lambda} \KL(\rho \vert\vert \pi) + \Upsilon^I(\lambda)
% \]
% where 
% \[\Upsilon^I(\lambda) \coloneqq \frac{1}{\lambda}\ln \E_{P \sim \calP} \exp\left(
% \calL(P, \dots,P, \calT) -  \tilde{\calL}(P, \dots, P, \calD_1, \dots, \calD_n)
% \right).\] 
% We calculate the KL-divergence term,
% \begin{align*}
%     \KL(\rho \vert \pi) & = \sum_{i=1}^n \KL(\calQ_i \vert\vert P).
% \end{align*}

% {\color{red}A few words about the sequence $P_1, \dots, P_n$ being independent: So for the case where one (offline learned) hyper-posterior is used for all tasks, this holds. Another way to go about it is to do some sort of forced exploration, such that we use different data points for each update $\calQ_i$. Or for instance, a ``forgetting'' strategy where we only look at the previous task for updating the hyper posterior. I think I might be able to relax this to history dependent and then bound the KL term using convexity of negative log \dots }
% {\color{blue} I'm also thinking about changing the setup to $\calQ$ being the same, but $Q_i = Q(S_{i-1},S_i,P_i)$. This probably makes more sense. }

==> content/supplement_dumps.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bounding the moment generating function with squared loss}
Assumptions:
\begin{itemize}
\item regression problem with $\calX \times \calY \subset \R^d \times \R$
\item family of linear predictors: $\calH = \{ h_{\bw}(\bx) = \bw \cdot \bx ~| ~ \bw \in \R^d \} $ 
\item Gaussian prior $P_{\mu_P, \sigma^2_P} = \calN(\mu_P, \sigma^2_P \bI)$
\item Gaussian hyper-prior $\calP(\mu_p) = \calN(0, \sigma^2_{\calP} \bI)$
\end{itemize}

Data generating process:
\begin{itemize}
\item $\bw_i^* \sim \calN(\mu_\calT, \sigma^2_\calT \bI)$
\item $\bx \sim p(\bx) = \calN(0, \sigma_{\bx}^2)$ 
\item $y = \bw_i^* \cdot \bx + \epsilon$ where $\epsilon \sim \calN(0, \sigma_{\epsilon}^2)$. Thus, we can write the conditional label distribution as $p_{\bw_i^*}(y|\bx) = \calN(\bw_i^* \cdot \bx, \sigma_{\epsilon}^2)$. Accordingly, the data distribution follows as $\calD_i = p(\bx) p_{\bw_i^*}(y|\bx)$.
\end{itemize}

We study negative log-likelihood $l(\bw, \bx, y) = \frac{1}{2} \ln(2\pi \sigma^2) + \frac{1}{2\sigma^2}(\bw \cdot \bx - y)^2$.


\paragraph{Bounding $\Upsilon^{\rom{1}}(\lambda)$:}

To show that the random variable $V_i = \calL(h, \calD_i) - l(h, z) = \E_{(\bx, y) \sim \calD_i} \left[ l(\bw, \bx, y) \right]- l(\bw, \bx, y)$ is sub-gamma, we need to find values $s > 0$ and $c \geq 0$ such that
%
\begin{equation}
\Upsilon^{\rom{1}}(\lambda) = \ln \E e^{\lambda V_i} \leq \frac{\lambda^2 s^2}{2(1-\lambda c) } ~, \quad \forall \lambda \in (0, \frac{1}{c}) ~.
\end{equation} 

 
\begin{align}
\Upsilon^{\rom{1}}(\lambda) = & \ln \E_{(\bx, y)} \E_{\bw} \exp \left(  \lambda \left(  \E_{(\bx, y)} \left[ l(\bw, \bx, y) \right]- l(\bw, \bx, y) \right) \right) \\
\leq & \ln \E_{(\bx, y)} \E_{\bw}  \exp \left(  \frac{\lambda}{2\sigma^2} \E_{(\bx, y)} \left[ (\bw \cdot \bx - y)^2  \right] \right) \\
= & \ln \E_{\bw}  \exp \left( \frac{\lambda}{2\sigma^2} \E_{\bx} \E_{y|\bx} \left[ (\bw \cdot \bx - y)^2 \right] \right) \\
= & \ln \E_{\bw}  \exp \left( \frac{\lambda}{2\sigma^2} \E_{\bx} \left[ ( \bx (\bw - \bw^*_i))^2  \right] + \frac{\lambda \sigma_\epsilon^2}{2\sigma^2}  \right) \\
& \ln \E_{\bw}  \exp \left( \frac{\lambda \sigma_{\bx}^2}{2\sigma^2} ||\bw - \bw^*_i||^2  + \frac{\lambda \sigma_\epsilon^2}{2\sigma^2}  \right) \\
= & \ln \left( \left(1 - 2  \frac{\lambda \sigma_{\bx}^2}{2\sigma^2}(\sigma_P^2 + \sigma_\calP^2)\right)^{-d/2} + \exp \left( \frac{ \frac{\lambda \sigma_{\bx}^2}{2\sigma^2} ||\bw^*_i||^2}{1 - 2  \frac{\lambda \sigma_{\bx}^2}{2\sigma^2} (\sigma_P^2 + \sigma_\calP^2)} \right) \right) + \frac{\lambda \sigma_\epsilon^2}{2\sigma^2}  \\
\leq & \frac{d \frac{\lambda \sigma_{\bx}^2}{2\sigma^2} (\sigma_P^2 + \sigma_\calP^2)}{1 - 2 \frac{\lambda \sigma_{\bx}^2}{2\sigma^2} (\sigma_P^2 +  \sigma_\calP^2)}  + \frac{\frac{\lambda \sigma_{\bx}^2}{2\sigma^2} ||\bw^*_i||^2}{1 - 2 \frac{\lambda \sigma_{\bx}^2}{2\sigma^2}(\sigma_P^2 + \sigma_\calP^2)}  + \frac{\lambda \sigma_\epsilon^2}{2\sigma^2} \\
= & \frac{ \frac{\lambda \sigma_{\bx}^2}{\sigma^2} ||\bw^*_i||^2  +  d \frac{\lambda \sigma_{\bx}^2}{\sigma^2} (\sigma_P^2 + \sigma_\calP^2) +  \frac{\lambda \sigma_\epsilon^2}{\sigma^2} -   \lambda^2 \sigma_\epsilon^2  \frac{\sigma_{\bx}^2}{\sigma^2} (\sigma_P^2 + \sigma_\calP^2)}{2(1 -  \lambda \frac{ \sigma_{\bx}^2}{\sigma^2} (\sigma_P^2 + \sigma_\calP^2))} \\
= & \frac{ \lambda^2 \frac{2}{\lambda \sigma^2} \left(  \sigma_{\bx}^2 (||\bw^*_i||^2  +  d (\sigma_P^2 + \sigma_\calP^2)) + \sigma_\epsilon^2 (1 -  \lambda   \frac{\sigma_{\bx}^2}{\sigma^2} (\sigma_P^2 + \sigma_\calP^2))\right) }{2(1 - \lambda    \frac{\sigma_{\bx}^2}{\sigma^2} (\sigma_P^2 + \sigma_\calP^2))} \\
=& \frac{\sigma^2 s^2}{2(1-\lambda c)}
\end{align}

with $c =  \frac{\sigma_{\bx}^2}{\sigma^2} (\sigma_P^2 + \sigma_\calP^2)$ and $s^2 = \frac{1}{\lambda \sigma^2} \left(  \sigma_{\bx}^2 (||\bw^*_i||^2  +  d (\sigma_P^2 + \sigma_\calP^2)) + \sigma_\epsilon^2 (1 -   \lambda c) \right) $


\paragraph{Bounding $\Upsilon^{\rom{2}}(\gamma)$:}

To show that the random variable $V^{\rom{2}}:= \E_{(D,S)  \sim \calT} \left[ \calL (Q(P, S), \calD) \right] - \calL (Q(P, S_i), \calD_i )$ is {\em sub-gamma} we need to find values $s_{\rom{2}}^2 > 0$ and parameter $c_{\rom{2}} > 0$ such that 
\begin{equation}
\Upsilon^{\rom{2}}(\gamma) = \ln \E_{(\calD, S) \sim \calT} \E_{P \sim \calP} \left[ \exp \left( \gamma V^{\rom{2}} \right) \right] \leq   \exp \left(\frac{\gamma^2 s_{\rom{2}}^2}{2(1- c_{\rom{2}} \gamma)} \right) \quad \forall \gamma \in ( 0, 1 / c_{\rom{2}} )
\end{equation}

\begin{align}
\Upsilon^{\rom{2}}(\gamma) =& \ln \E_{(\calD, S) \sim \calT} \E_{P \sim \calP}  \left[ \exp \left( \gamma V^{\rom{2}} \right) \right] \\
\leq& \ln \E_{(\calD, S) \sim \calT} \E_{P \sim \calP} \left[ \exp \left( \frac{\gamma}{2\sigma^2}  \E_{(D,S)  \sim \calT} \E_{\bw \sim Q(P, S)} \left[\E_{\bx} \E_{y|\bx} \left[ (\bw \cdot \bx - y)^2 \right] \right] \right) \right] \\
= & \ln \E_{P \sim \calP} \left[ \exp \left( \frac{\gamma}{2\sigma^2}  \E_{(D,S)  \sim \calT} \E_{\bw \sim Q(P, S)} \E_{\bx} \E_{y|\bx} \left[ (\bw \cdot \bx - y)^2 \right]  \right) \right] \\
\leq & \ln \E_{P \sim \calP} \left[ \exp \left(\frac{\gamma}{2\sigma^2}  \E_{\bw^* \sim \calN(\mu_\calT, \sigma^2_\calT \bI)} \E_{\bw \sim P}\left[  \sigma_{\bx}^2||\bw - \bw^*||^2  + \sigma_\epsilon^2 \right]  \right) \right] \\
= & \ln \E_{\mu_P \sim \calP} \left[ \exp \left( \frac{\gamma}{2\sigma^2} (\sigma_{\bx}^2 (||\mu_\calT - \mu_P||^2 + \sigma_\calT^2 + \sigma_P^2) + \sigma_\epsilon^2) \right) \right] \\
= &  \ln \left( \left(1 - 2 \frac{\gamma}{2\sigma^2}  \sigma_{\bx}^2 \sigma_\calP^2)\right)^{-d/2} + \exp \left( \frac{\frac{\gamma}{2\sigma^2} \sigma_{\bx}^2 ||\mu_\calT||^2}{1 - 2 \frac{\gamma \sigma_{\bx}^2}{2\sigma^2}   \sigma_\calP^2} \right) \right) +\frac{\gamma  \sigma_{\bx}^2}{2\sigma^2}  (\sigma_\calT^2 + \sigma_P^2) + \frac{\gamma  \sigma_\epsilon^2}{2\sigma^2}  \\
\leq & \frac{d \frac{\gamma}{2\sigma^2} \sigma_{\bx}^2 \sigma_\calP^2}{1 - 2 \frac{\gamma}{2\sigma^2} \sigma_{\bx}^2 \sigma_\calP^2} + \frac{\frac{\gamma}{2\sigma^2} \sigma_{\bx}^2 ||\mu_\calT||^2}{1 - 2 \frac{\gamma}{2\sigma^2} \sigma_{\bx}^2 \sigma_\calP^2} + \frac{\gamma}{2\sigma^2}(\sigma_{\bx}^2 (\sigma_\calT^2 + \sigma_P^2) + \sigma_\epsilon^2) \\
=& \frac{d \frac{\gamma}{\sigma^2} \sigma_{\bx}^2 \sigma_\calP^2 + \frac{\gamma}{\sigma^2}\sigma_{\bx}^2 ||\mu_\calT||^2 + (1 - 2 \gamma \frac{\sigma_{\bx}^2 \sigma_\calP^2}{\sigma^2}) \frac{\gamma}{\sigma^2} (\sigma_{\bx}^2 (\sigma_\calT^2 + \sigma_P^2) + \sigma_\epsilon^2)}{ 2 (1 - \gamma \frac{\sigma_{\bx}^2 \sigma_\calP^2}{\sigma^2} )} \\
=& \frac{\gamma^2 \left( \frac{1}{\gamma \sigma^2}( \sigma_{\bx}^2 (||\mu_\calT||^2 + d  \sigma_\calP^2) + (1 - \gamma c ) (\sigma_{\bx}^2 (\sigma_\calT^2 + \sigma_P^2) + \sigma_\epsilon^2) \right)}{2(1 - \gamma c)}\\
=&  \frac{\gamma^2 s^2}{2(1 - \gamma c)}
\end{align}

with $c = \frac{\sigma_{\bx}^2 \sigma_\calP^2}{\sigma^2}$ and $s^2=\frac{1}{\gamma \sigma^2}( \sigma_{\bx}^2 (||\mu_\calT||^2 + d  \sigma_\calP^2) + (1 - \gamma c ) (\sigma_{\bx}^2 (\sigma_\calT^2 + \sigma_P^2) + \sigma_\epsilon^2)$



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Second attempt bounding quadratic loss}

\paragraph{Bounding $\Upsilon^{\rom{1}}(\lambda)$:}

To show that the random variable $V_i = \calL(h, \calD_i) - l(h, z) = \E_{(\bx, y) \sim \calD_i} \left[ l(\bw, \bx, y) \right]- l(\bw, \bx, y)$ is sub-gamma, we need to find values $s > 0$ and $c \geq 0$ such that
%
\begin{equation}
\Upsilon^{\rom{1}}(\lambda) = \ln \E e^{\lambda V_i} \leq \frac{\lambda^2 s^2}{2(1-\lambda c) } ~, \quad \forall \lambda \in (0, \frac{1}{c}) ~.
\end{equation} 

 
\begin{align}
\Upsilon^{\rom{1}}(\lambda) = & \ln \E_{\bw} \E_{(\bx, y)} \exp \left(  \lambda \left(  \E_{(\bx, y)} \left[ l(\bw, \bx, y) \right]- l(\bw, \bx, y) \right) \right) \\
= & \ln \E_{\bw} \E_{(\bx, y)}  \exp \left(\lambda \left( \sigma_{\bx}^2 ||\bw - \bw^*_i||^2  + \sigma_\epsilon^2 -  (\bw \cdot \bx - y)^2  \right) \right) \\
= & \ln \E_{\bw} \E_{\bx} \E_{\epsilon}   \exp \left(\lambda \left( \sigma_{\bx}^2 ||\bw - \bw^*_i||^2  + \sigma_\epsilon^2 -  (\bw \cdot \bx - \bw^*_i \cdot \bx + \epsilon)^2  \right) 
 \right) \\ 
 = & \ln  \E_{\bw} \E_{\bx} \E_{\epsilon} \exp \left(\lambda \left( \sigma_{\bx}^2 ||\bw - \bw^*_i||^2  + \sigma_\epsilon^2 -  ((\bw - \bw^*_i) \cdot \bx  + \epsilon)^2  \right) 
 \right) \\
  = & \ln  \E_{\bw} \left[ \exp \left(\lambda \left( \sigma_{\bx}^2 ||\bw - \bw^*_i||^2  + \sigma_\epsilon^2 \right) \right)  \underbrace{\E_{\bx} \E_{\epsilon} \exp \left( -  ((\bw - \bw^*_i) \cdot \bx  + \epsilon)^2\right)}_{(*)}  \right] \label{eq:log_laplace_1}
\end{align}


\begin{align}
(*) = & \E_{\bx} \E_{\epsilon}  \exp \left(- \lambda ((\bw - \bw^*_i) \cdot \bx  + \epsilon)^2  \right) \\
= &(1 + 2\lambda \sigma^2_\epsilon)^{-\frac{1}{2}} \E_{\bx}  \exp \left( - \frac{\lambda ((\bw - \bw^*_i) \cdot \bx )^2}{1 + 2\lambda \sigma^2_\epsilon} \right) \\
= &(1 + 2\lambda \sigma^2_\epsilon)^{-\frac{1}{2}} \E_{\bx}  \exp \left( - \frac{\lambda}{1 + 2\lambda \sigma^2_\epsilon} ((\bw - \bw^*_i) \cdot \bx )^2 \right) \\
= &(1 + 2\lambda \sigma^2_\epsilon)^{-\frac{1}{2}} (1 + 2 \frac{\lambda}{1 + 2\lambda \sigma^2_\epsilon} ||\bw - \bw^*_i||^2 \sigma^2_\bx)^{-\frac{1}{2}} \\
= &(1 + 2\lambda \sigma^2_\epsilon + 2\lambda ||\bw - \bw^*_i||^2 \sigma^2_\bx)^{-\frac{1}{2}} \label{eq:second_mgf_term_closed_form}
\end{align}

Now, we can insert (\ref{eq:second_mgf_term_closed_form}) into (\ref{eq:log_laplace_1})


\begin{align}
\Upsilon^{\rom{1}}(\lambda) = & \ln  \E_{\bw \sim \calN(0,\sigma_P^2 I_d)} \left[ \frac{\exp \left(\lambda \left( \sigma_{\bx}^2 ||\bw - \bw^*_i||^2  + \sigma_\epsilon^2 \right) \right)}{(1 + 2\lambda \sigma^2_\epsilon + 2\lambda \sigma^2_\bx ||\bw - \bw^*_i||^2 )^{\frac{1}{2}}} \right] \\
\leq &  \lambda \left( \sigma_{\bx}^2 ||\bw^*_i||^2  + \sigma_\epsilon^2 \right) + \ln  \E_{\bw \sim \calN(0,\sigma_P^2 \bI_d)} \left[ \frac{\exp \left(\lambda  \sigma_{\bx}^2 ||\bw||^2  \right)}{(1 + 2\lambda \sigma^2_\epsilon + 2\lambda \sigma^2_\bx ||\bw - \bw^*_i||^2 )^{\frac{1}{2}}} \right]\\
\leq &  \lambda \left( \sigma_{\bx}^2 ||\bw^*_i||^2  + \sigma_\epsilon^2 \right) + \ln  \E_{w \sim \calN(0,\sigma_P^2)} \left[ \frac{\exp \left(\lambda  \sigma_{\bx}^2 d w^2  \right)}{(1 + 2\lambda \sigma^2_\epsilon + 2\lambda \sigma^2_\bx ||\bw^*_i||^2 + 2 \lambda \sigma_{\bx}^2 d w^2)^{\frac{1}{2}}} \right] \label{eq:345345}
\end{align}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma} \label{lemma:bound_bessel}
Let $a, b \in \R^+ $ and $x \sim \calN(0, \sigma^2)$ be a Gaussian random variable with mean $0$ and variance $ \sigma^2$. Then, we have
\begin{equation}
\E_{x \sim \calN(0, \sigma^2)} \left[ \frac{e^{a x^2}}{(b + 2ax^2 )^{\frac{1}{2}}} \right] < \frac{1}{(b -2 b a \sigma^2 ))^{\frac{1}{2}}}
\end{equation}
\end{lemma}
\begin{proof}
\begin{equation}
E_{x \sim \calN(0, \sigma^2)} \left[ \frac{e^{a x^2}}{(b + 2ax^2 )^{\frac{1}{2}}} \right] = \frac{e^{\frac{b}{8} \left(\frac{1}{a \sigma^2}-2\right)} K_0\left(\frac{b}{8} \left(\frac{1}{a \sigma^2}-2\right)\right)}{\sqrt{4 a \pi \sigma^2 }} \label{eq:closed_form_expectation_mgf_bessel}
\end{equation}
wherein $K_v(y)$ is the modified Bessel function of the second kind.  In particular, for $v=0$ we have
\begin{equation}
K_0(y) = \int_0^\infty e^{-y \cosh(t)}dt < \frac{\sqrt{\pi} e^{-y}}{\sqrt{2y}} \label{eq:upper_bound_bessel}
\end{equation}
For a proof of the inequality in (\ref{eq:upper_bound_bessel}), we refer to \citet{yang2017approximating}. Using (\ref{eq:upper_bound_bessel}) to upper-bound (\ref{eq:closed_form_expectation_mgf_bessel}), we obtain
\begin{align}
E_{x \sim \calN(0, \sigma^2)} \left[ \frac{e^{a x^2}}{(b + 2ax^2)^{\frac{1}{2}}} \right] <& \frac{1}{\sqrt{ b (1 -2 a \sigma^2 ) }}
\end{align}
which concludes the proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next, we invoke Lemma \ref{lemma:bound_bessel} with $a=\lambda \sigma_{\bx}^2 d$ and $b= 1 + 2\lambda \sigma^2_\epsilon + 2\lambda \sigma^2_\bx ||\bw^*_i||^2 $  


\begin{align}
(\ref{eq:345345}) < &  \lambda \left( \sigma_{\bx}^2 ||\bw^*_i||^2  + \sigma_\epsilon^2 \right) - \frac{1}{2}\ln \left(b (1 -2 a \sigma_P^2) \right) \\
 = &  \lambda \underbrace{\left( \sigma_{\bx}^2 ||\bw^*_i||^2  + \sigma_\epsilon^2 \right)}_{\vartheta} - \frac{1}{2}\ln \left((1 + 2 \lambda \underbrace{\left( \sigma_{\bx}^2 ||\bw^*_i||^2  + \sigma_\epsilon^2 \right)}_{\vartheta}) (1 -2 \lambda d \sigma_{\bx}^2 \sigma_P^2) \right) \\
  = &  \lambda \vartheta - \frac{1}{2}\ln \left((1 + 2 \lambda \vartheta - 2 \lambda d \sigma_{\bx}^2 \sigma_P^2 - 4 \lambda^2 d  \sigma_{\bx}^2 \sigma_P^2 \vartheta \right) \\
 < & \lambda \vartheta + \frac{ \lambda d \sigma_{\bx}^2 \sigma_P^2 +  2 \lambda^2 d  \sigma_{\bx}^2 \sigma_P^2 \vartheta - \lambda \vartheta}{1 + 2 \lambda \vartheta - 2 \lambda d \sigma_{\bx}^2 \sigma_P^2 - 4 \lambda^2 d  \sigma_{\bx}^2 \sigma_P^2 \vartheta } \\
  = & \lambda \vartheta + \frac{ \frac{\lambda}{2}  c}{1 - \lambda c } \\ 
  = & \frac{\lambda^2 \left( 2 \vartheta (\frac{1}{\lambda} - c) + \frac{c}{\lambda}   \right)}{2(1 - \lambda c) } 
\end{align}

where $c =   2 d \sigma_{\bx}^2 \sigma_P^2 + 4 \lambda d  \sigma_{\bx}^2 \sigma_P^2 \vartheta - 2 \vartheta$




==> content/supplement_playground.tex <==
\section{Revised Proof of Bounding the CGFs}
    Finally, we aim to bound the random quantity $\frac{1}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{1}{\lambda} \Upsilon^\rom{2}(\lambda)$. Note that the randomness of $\Upsilon^{\rom{1}}(\gamma)$ is governed by the random data points $z_{i,j}$ sampled i.i.d.\ from the respective data distribution $\calD_i$, while $\Upsilon^\rom{2}(\lambda)$ is governed by random tasks sampled from the environment $\calT$. 
    
    First, we factor out $\sqrt{n}$ from $\gamma$ and $\lambda$, obtaining
    \begin{equation} \label{eq:factor_out_sqrt_n}
    \frac{1}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{1}{\lambda} \Upsilon^\rom{2}(\lambda) = \frac{1}{\sqrt{n}} \left( \frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda) \right)
    \end{equation}
    Next, we proceed by bounding the inner part on the RHS, i.e., $\frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda)$. Using Markov's inequality, we have 
    %
    \begin{equation}
    e^{\frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda)}  \leq  \frac{\E \left[ e^{ \frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda)} \right]}{\delta}
    \end{equation}
    and thus
    \begin{equation} \label{eq:high_prob_bound_generic}
     \frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda) \leq \log \E \left[ e^{ \frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda)} \right] - \log \delta
\end{equation}
with probability at least $1-\delta$. Next, we bound the expectation, i.e., 

\begin{align} \label{eq:dskjfkjsdfb}
\E \left[ e^{ \frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda)} \right] = ~ \E_\calT \left[ e^{\frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda)}  ~ \E_{\calD_1} ... \E_{\calD_1} \left[  \left(e^{\Upsilon^{\rom{1}}(\gamma)}\right)^{\frac{\sqrt{n}}{\gamma} } \right] \right] ~. 
\end{align}
%
If $\gamma \geq \sqrt{n}$, $x \mapsto x^{\sqrt{n}/\gamma}$ is a concave function, we can obtain an upper bound on (\ref{eq:dskjfkjsdfb}) by using Jensen's inequality to move the exponent in (\ref{eq:dskjfkjsdfb}) outside the inner expectation. Further, we denote $V_i^\rom{2} := \E_{\calT} \left[ \calL (Q_i, \calD)  \right] - \calL(Q_i, \calD_i )$ as i.i.d.\ realizations of the random variable under the task distribution.  Similarly, for each $i=1, ....,n$ and $j=1,....,m$, we denote the independent realizations of $\calL(h, \calD_i) - l(h, z_{ij})$ as $V_{ij}^\rom{1}$. Hence, we can write 
\begin{align} 
    (\ref{eq:dskjfkjsdfb}) \leq & ~ \E_\calT \left[ e^{\frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda)}  ~ \E_{\calD_1} ... \E_{\calD_1} \left[ e^{\Upsilon^{\rom{1}}(\gamma)} \right]^{\frac{\sqrt{n}}{\gamma}} \right] \\
    = & ~ \E_\calT \bigg[ \E_{\calP} \left[ e^{\frac{\lambda}{n} \sum_{i=1}^n V_i^{\rom{2}}} \right]^{\sqrt{n}/\lambda}  \cdot  \E_{\calP} \E_{P}  \E_{\calD_1} ... ~\E_{\calD_n} \left[ e^{ \frac{\gamma}{nm} \sum_{i=1}^n \sum_{j=1}^m V_{ij}^{\rom{1}}}\right]^{\sqrt{n}/\gamma}  \bigg] \\
    = & ~ \E_\calT \bigg[ \E_{\calP} \left[ \prod_{i=1}^n e^{\frac{\lambda}{n}  V_i^{\rom{2}}} \right]^{\sqrt{n}/\lambda}  \cdot \E_{\calP} \E_{P}  \E_{\calD_1} ... ~\E_{\calD_n} \left[  \prod_{i=1}^n \prod_{j=1}^m  e^{ \frac{\gamma}{nm} V_{ij}^{\rom{1}}}\right]^{\sqrt{n}/\gamma}  \bigg] ~.
\end{align}

Following the arguments of \citet[][Proof of Corollary 4]{germain2016pac}, we obtain
\begin{align} \label{eq:dskjfkljsbldkzbf}
    (\ref{eq:dskjfkjsdfb})  \leq ~ &  \E_\calT  \bigg[ \prod_{i=1}^n \E_{\calP} \left[  e^{\frac{\lambda}{n} V_i^\rom{2}} \right]^{\sqrt{n}/\lambda}   \left( \prod_{i=1}^n \prod_{j = 1}^{m} \E_{\calP} \E_{P}  \E_{\calD_i} e^{ \frac{\gamma}{nm} V_{ij}^\rom{1}}\right)^{\sqrt{n}/\gamma}  \bigg] ~.
\end{align}

\paragraph{Case I: bounded loss}
First, we bound the moment-generating function (MGF) corresponding to $\Upsilon^{\rom{1}}(\gamma)$.
If the loss function $l(h_i, z_{ij})$ is bounded in $[a,b]$, we can apply Hoeffding's lemma to the moment generating function on the right of (\ref{eq:dskjfkljsbldkzbf}), obtaining:
\begin{align}
     \E \left[ e^{ \frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda)} \right]  \leq ~ & 
    \E_\calT \bigg[ \E_{\calP} \left[ \prod_{i=1}^n e^{\frac{\lambda}{n} V_i^\rom{2}} \right]^{\sqrt{n}/\lambda}  \left( \prod_{i=1}^n \prod_{j = 1}^{m} e^{\frac{\gamma^2  (b-a)^2}{8 n^2 m^2}} \right)^{\sqrt{n}/\gamma} \bigg] \\
     = ~ & \E_\calT \bigg[ \E_{\calP} \left[ \prod_{i=1}^n e^{\frac{\lambda}{n} V_i^\rom{2}} \right]^{\sqrt{n}/\lambda}  \bigg]  ~ e^{\frac{\gamma  (b-a)^2}{8 \sqrt{n} m}}
\end{align}
Crucially, the upper bound $e^{\frac{\gamma  (b-a)^2}{8 \sqrt{n} m}} \geq \E_{\calD_1} ... \E_{\calD_1} \left[  \left(e^{\Upsilon^{\rom{1}}(\gamma)}\right)^{\frac{\sqrt{n}}{\gamma} } \right]$ no longer depends on the tasks which are sampled from $\calT$ which allows us to move it outside the expectation under $\calT$.
In the second step, we follow analogous steps to bound the MGF corresponding to $\Upsilon^\rom{2}(\lambda)$. Again, assuming that $\lambda > \sqrt{n}$, we use Jensen's inequality to move the exponent outside of the outer expectation and follow the arguments of \citet[][Proof of Corollary 4]{germain2016pac} to obtain
\begin{align}
     \E \left[ e^{ \frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda)} \right]  \leq ~ & e^{\frac{\gamma  (b-a)^2}{8 \sqrt{n} m}}  \left[ \prod_{i=1}^n \E_\calT \E_{\calP}  e^{\frac{\lambda}{n} V_i^\rom{2}} \right]^{\sqrt{n}/\lambda} ~.
\end{align}
From the boundedness of the loss together with Hoeffding's inequality, it follows that
\begin{align}
     \E \left[ e^{ \frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda)} \right]  \leq ~ & e^{\frac{\gamma (b-a)^2}{8 \sqrt{n} m} + \frac{\lambda (b-a)^2}{8 \sqrt{n} }} \label{eq:kjdnkjnsdf}
\end{align}
Finally, we insert (\ref{eq:kjdnkjnsdf}) into (\ref{eq:high_prob_bound_generic}) and set $\gamma = n \beta$ to obtain that
\begin{align}
\frac{1}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{1}{\lambda} \Upsilon^\rom{2}(\lambda)
\leq  \left( \frac{\beta}{8  m} + \frac{\lambda}{8 n} \right)  (b-a)^2 - \frac{1}{\sqrt{n}} \ln \delta
\end{align}
with probability at least $1-\delta$ which concludes our high-probability bound on the CGFs in case of a bounded loss.

\paragraph{Case II: sub-gamma loss} First, we bound the moment-generating function (MGF) corresponding to $\Upsilon^{\rom{1}}(\gamma)$. If the loss is sub-gamma with variance factor $s_{\rom{1}}^2$ and scale parameter $c_{\rom{1}}$ under the two-level prior and any data distribution $\calD$ in the support of $\calT$, i.e., 
\begin{equation}
    \E_{P \sim \calP} \E_{h \sim P}  \E_{z \sim \calD} \left[ e^{\nu (\calL(\calD, h) - l(h, z)) } \right] \leq \exp \left( \frac{\nu^2 s_{\rom{1}}^2}{2(1- \nu c_{\rom{2}})} \right) ~~ \forall ~ \nu \in (0, 1 / c_{\rom{1}})
\end{equation}
then, with $\nu := \gamma / (nm)$, we have that, if $\gamma < \frac{mn}{c_{\rom{1}}}$,
\begin{align}
    \E \left[ e^{ \frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda)} \right] 
     & \leq \E_\calT  \bigg[ \prod_{i=1}^n \E_{\calP} \left[  e^{\frac{\lambda}{n} V_i^\rom{2}} \right]^{\sqrt{n}/\lambda}   \left( \prod_{i=1}^n \prod_{j = 1}^{m} \exp \left( \frac{\gamma^2 s_{\rom{1}}^2}{2 n^2 m^2(1-\frac{c_{\rom{1}}  \gamma}{nm})} \right) \right)^{\sqrt{n}/\gamma}  \bigg] \\
     & = \prod_{i=1}^n \E_\calT \E_{\calP} \left[  e^{\frac{\lambda}{n} V_i^\rom{2}} \right]^{\sqrt{n}/\lambda}   \exp \left( \frac{\gamma s_{\rom{1}}^2}{2 \sqrt{n}  m (1- \frac{ c_{\rom{1}} \gamma}{nm})} \right) \label{eq:dksjfbkjsdfsk}
\end{align}
Second, we bound the remaining moment-generating function (MGF) corresponding to $\Upsilon^{\rom{2}}(\lambda)$. For that, we use the assumption that the random variable $V_i^\rom{2} := \E_{\calT} \left[ \calL (Q_i, \calD)  \right] - \calL(Q_i, \calD_i )$ is sub-gamma with variance factor $s_{\rom{2}}^2$ and scale parameter $c_{\rom{2}}$ under the hyper-prior $\calP$ and the task distribution $\calT$. That is, its moment generating function can be bounded by that of a Gamma distribution $\Gamma(s_{\rom{2}}^2, c_{\rom{2}})$:
\begin{equation}
 \E_{(\calD, S) \sim \calT} \E_{P \sim \calP} \left[  e^{\kappa  \E_{(D,S)  \sim \calT} \left[ \calL (Q(P, S), \calD) \right] - \calL (Q(P, S), \calD )}\right] \leq   \exp \left(\frac{\kappa^2 s_{\rom{2}}^2}{2(1- c_{\rom{2}} \kappa)} \right) ~ \forall \kappa \in ( 0, 1 / c_{\rom{2}} ) ~.
\end{equation}
Using the sub-gamma assumption with $\kappa := \lambda / n$, we can further bound (\ref{eq:dskjfkjsdfb}) as:
\begin{equation}
     \E \left[ e^{ \frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda)} \right]  \leq \exp \left( \frac{\lambda s^2_{\rom{2}}}{2 \sqrt{n} (1 - \frac{\lambda c_{\rom{2}}}{n})} \right)   \exp \left( \frac{\gamma s_{\rom{1}}^2}{2 \sqrt{n}  m (1- \frac{ c_{\rom{1}} \gamma}{nm})} \right) ~; \label{eq:kjndf2832ksdjcjsd}
\end{equation}
under the condition that $\lambda < \frac{n}{c_{\rom{2}}}$.

Finally, we insert (\ref{eq:kjndf2832ksdjcjsd}) into (\ref{eq:high_prob_bound_generic}) and set $\gamma = n \beta$ to obtain that
\begin{align}
\frac{1}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{1}{\lambda} \Upsilon^\rom{2}(\lambda)
\leq  \frac{\beta s_{\rom{1}}^2}{2  m (1- \frac{ c_{\rom{1}} \beta}{m})} + \frac{\lambda s^2_{\rom{2}}}{2 n (1 - \frac{\lambda c_{\rom{2}}}{n})} - \frac{1}{\sqrt{n}} \log \delta
\end{align}
with probability at least $1-\delta$ which concludes our high-probability bound on the CGFs in the case of sub-gamma tail assumptions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% \subsection{Bounding the CGFs separately}
% \lemma{}
% \begin{equation} \label{eq:factor_out_sqrt_n}
% \frac{1}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{1}{\lambda} \Upsilon^\rom{2}(\lambda) = \frac{1}{\sqrt{n}} \left( \frac{\sqrt{n}}{\gamma} \Upsilon^{\rom{1}}(\gamma) +  \frac{\sqrt{n}}{\lambda} \Upsilon^\rom{2}(\lambda) \right)
% \end{equation}


% By the independence of the samples, the boundedness of $l \in [a, b]$ and Hoeffding's lemma, we can bound the MGF as follows:
% \begin{align}
% & \E_{\calD_1}, ..., \E_{\calD_n} \E_{\calP} \E_{h \sim P} \left[ e^{  \frac{\gamma}{n} \sum_{i=1}^n \calL(h, \calD_i) - \hat{\calL}(h, S_i)}  \right] \\
% = & \E_{\calP} \E_{h \sim P} \E_{\calD_1}, ..., \E_{\calD_n} \left[ \prod_{i}^n \prod_{i}^{m_i} e^{ \frac{\gamma}{nm_i} (\calL(h, \calD_i) - l(h, z_{ij}) )} \right] \\
% = &  \prod_{i=1}^n \prod_{j=1}^{m_i} \E_{z_{ij} \sim \calD_i} \left[ e^{ \frac{\gamma}{nm_i} (\calL(h, \calD_i) - l(h, z_{ij}) )} \right]  \\
% \leq & \prod_{i=1}^n \prod_{j=1}^{m_i}  e^{ \frac{\gamma^2}{n^2 m_i^2} \frac{(b-a)^2}{8}} \\
% = & e^{ \frac{\gamma^2}{n m} \frac{(b-a)^2}{8}} ~.
% \end{align}

% Using Markov's inequality, we have with probability at least $1-\delta$ that
% \begin{align}
% &  \frac{1}{\gamma} \ln \E_{\calP} \E_{h \sim P} \left[ e^{  \frac{\gamma}{n} \sum_{i=1}^n \calL(h, \calD_i) - \hat{\calL}(h, S_i)}  \right] \\
% \leq &  \frac{\gamma}{n m} \frac{(b-a)^2}{8} - \frac{1}{\gamma} \ln(\delta)
% \end{align}
